Prompt2NeRF-PIL: Fast NeRF Generation via Pretrained Implicit Latent

This paper explores promptable NeRF generation (e.g., text prompt or single image prompt) for direct conditioning and fast generation of NeRF parameters for the underlying 3D scenes, thus undoing complex intermediate steps while providing full 3D generation with conditional control. Unlike previous diffusion-CLIP-based pipelines that involve tedious per-prompt optimizations, Prompt2NeRF-PIL is capable of generating a variety of 3D objects with a single forward pass, leveraging a pre-trained implicit latent space of NeRF parameters. Furthermore, in zero-shot tasks, our experiments demonstrate that the NeRFs produced by our method serve as semantically informative initializations, significantly accelerating the inference process of existing prompt-to-NeRF methods. Specifically, we will show that our approach speeds up the text-to-NeRF model DreamFusion and the 3D reconstruction speed of the image-to-NeRF method Zero-1-to-3 by 3 to 5 times.

==> sec/2_related_work.tex <==
\section{Related Works}
\textbf{Neural Radiance Field.}\quad NeRF, or Neural Radiance Field  introduced in~\cite{mildenhall2021nerf} is a generative model that establishes a mapping from accurate camera poses to a 3D scene given a set of images. Unlike traditional representations such as voxels and meshes which highly depend on explicit 3D models, the foundation of NeRF is a radiance field, which is a function of how a batch of light rays travels through a 3D volume.
NeRF can be formulated as:
\begin{align*}
    F:(\textbf{x}, \textbf{d}) \rightarrow (\textbf{c}, \boldsymbol{\sigma})
\end{align*}
where ${\bf x}=(x,y,z)$, ${\bf d}=(\Theta,\phi)$ are respectively the location coordinate and direction in a predefined space, ${\bf c}=(r,g,b)$ is the color at the position, and $\boldsymbol{\sigma}$ can be thought of the probability that a light ray is occluded in 3D space.
Following this novel representation, 
%many modifications achieved satisfying performance. 
Mip-NeRF~\cite{barron2021mip} alternatively uses light cones to reduce artifacts, and Bungee-NeRF~\cite{xiangli2022bungeenerf} uses multi-resolution images to train Mip-NeRF progressively, which enables city-scale scenes rendering. Existing works also use explicit representations to obtain a hybrid NeRF. For example, Instant-NGP~\cite{muller2022instant} uses a multi-resolution hash encoding structure; TensoRF~\cite{chen2022tensorf} adopts factorizations to achieve a compact encoding space; Plenoxels~\cite{yu_and_fridovichkeil2021plenoxels} leverages a sparse grid for NeRF synthesis. In this experimental work, we adopt the MLP similarly done in the first NeRF work~\cite{mildenhall2021nerf} as the foundation model in coarse-to-fine refinement.

\noindent\textbf{Variational AutoEncoders.}\quad The Variational Autoencoder (VAE)~\cite{kingma2013auto} 
%is specially designed for generative modeling tasks to 
learns a low-dimensional latent space to encode the underlying distribution of the input data, thus allowing sampling from the latent to enable the generative feature. 
%{\color{blue} LJM: mention other improvements. } 
VAE demonstrates robustness in handling noisy data, thus, in this work, we leverage its inherent properties that facilitate smooth interpolation between latent variables, so that meaningful semantic relationships can be preserved. 
% {\color{blue} LJM: need to mention this? How to explain it's old but we still use it?}
\begin{comment}
    
\noindent \textbf{2D Diffusion Models.}\quad Diffusion Probabilistic models {\color{blue} LJM: add cites here} have become a popular choice for generative modeling due to their superior performance compared to their predecessors. These models have demonstrated better image synthesis capabilities than GANs~\cite{goodfellow2014generative}, not only in terms of quality and fidelity but also in  text-conditioning capability. In particular, Latent Diffusion~\cite{rombach2022highresolution} can generate high-resolution images by applying diffusion in the latent space of pretrained autoencoders.

\noindent \textbf{Adding control to diffusion model.}\quad The emergence of diffusion models has prompted many works  on fine-tuning pre-trained diffusion models on custom datasets, which enables custom image generation from user-supplied prompts while preserving the original generation capabilities. Examples include Text Inversion~\cite{gal2022image}, LoRA~\cite{hu2021lora}, DreamBooth~\cite{ruiz2023dreambooth}, and ControlNet~\cite{zhang2023adding}. In our work, we utilize Controlnet to finetune pre-trained stable diffusion checkpoints to enhance output quality. This paper employs a rectified latent diffusion model for NeRF refinement. 
\end{comment}

% \noindent \textbf{CLIP} \quad Contrastive Language-Image Pre-Training, or CLIP, plays a significant role in our approach, as it offers a zero-shot capability that bridges gap between the latent spaces of text and image. To date, pre-trained CLIP has been utilized for various zero-shot downstream applications~\cite{luo2021clip4clip, fang2021clip2video, lei2021more, sanghi2022clipforge}. %Among them, CLIP-Forge~\cite{sanghi2022clipforge} utilizes pre-trained CLIP as a text encoder to extract texture and structural information from text and generate mesh 3D models. 
% Our approach involves pairing an implicit NeRF latent space with CLIP features, providing the ability to generate NeRF models from a single text prompt.

\noindent \textbf{CLIP and CLIP-Based 3D Generation} \quad Contrastive Language-Image Pre-Training (CLIP)~\cite{radford2021learning} offers a zero-shot capability that bridges the gap between the latent spaces of text and image. To date, it has been utilized for various zero-shot downstream applications~\cite{luo2021clip4clip, fang2021clip2video, lei2021more, sanghi2022clipforge}. As CLIP bridges text and vision, many works~\cite{sanghi2022clipforge, wang2022clip, jang2021codenerf, michel2022text2mesh, wang2023nerf} attempt to use it to optimize 3D models. However, despite their innovations, most of these works require a considerable amount of time to achieve satisfactory results. Recently, an image-to-3D work Zero-1-to-3~\cite{liu2023zero1to3} tweaks Stable Diffusion~\cite{rombach2022highresolution} to adopt a vector that combines clip image embedding and pose information as input, and employs the images generated by their model as input to train NeRF model. Other methods such as~\cite{poole2022dreamfusion, lin2023magic3d} have attempted to leverage the vast information within pretrained generative models via score distillation sampling under CLIP's guidance, by incorporating Stable Diffusion. Though having better performances on zero-shot generations, these approaches still require a long time for self-optimization and suffer from poor view consistency due to the use of 2D supervision without any initialization or view information. Therefore, aligning CLIP's embedding space with the 3D structure space is necessary.%, and that is precisely what we have attempted to do.

\noindent \textbf{Concurrent Works}\quad At the time of writing, we noticed one concurrent work\footnote{Concurrent works to CVPR'24 submission (November 2023) include ICCV'23 (October), NeurIPS'23 (December). For arXiv, see CVPR'24 submission policy and FAQ.} also investigates the ability to implicitly generate NeRF structures. ATT3D~\cite{lorraine2023att3d}, which adopts the InstantNGP~\cite{muller2022instant} NeRF backbone, optimizes a set of prompts at the same time to save training time and share the feature between the prompts to enables unseen generation. However, the amortization direction is quite limited as the result figures shown in the paper, and that the implicit part only lies in the feature grid of InstantNGP. Other text-to-3D models such as~\cite{shi2023mvdream,wang2023prolificdreamer} aim to solve the 3D consistency problem whose setting is thus different from ours.


==> sec/X_suppl_ours.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

\section{Rotation-invariant Mapping}
\label{sec:supp-rotation-invariant}

As mentioned in Sec.\ 3.2, %~\cref{sec:method-pipeline}
here, we demonstrate that by randomly selecting images from different viewpoints during the semantic alignment training, our model can learn a rotation-invariant mapping, i.e., from a general semantic representation invariant to viewpoint and rotation to the implicit NeRF ~\cite{mildenhall2021nerf} parameter space.

% \Cref{fig:supp-rot-inv} shows the comparisons. {\color{red} Add some descriptions/conclusions similar to the caption} 
The presented findings can be observed in~\cref{fig:supp-rot-inv}. The upper section of the figure exhibits eight images, each representing inference results obtained from randomly selected viewpoints. These images demonstrate a high degree of similarity, indicating consistent outcomes across different viewpoints. Conversely, in the lower section of the figure, only the first image, which derived from the training viewpoint, depicts satisfactory results. However, when inferring from alternative viewpoints, the generated outcomes lack consistency and fail to align with the desired expectations.
To ensure fairness, the two checkpoints we used for comparison were trained to similar accuracies, with the fixed-view checkpoint having a slightly higher accuracy since it is more stable during training.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/rand-1.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/rand-2.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/rand-3.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/rand-4.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/rand-5.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/rand-6.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/rand-7.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/rand-8.png}\\
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/norand-1.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/norand-2.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/norand-3.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/norand-4.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/norand-5.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/norand-6.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/norand-7.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/rot-invar/green-chair/norand-8.png}
    \caption{Comparison of inference results when using randomly-selected views (top) and fixed view (bottom) during semantic alignment. The results in column $i$, $i=1,2,\cdots 8$ are obtained by using the clip embedding of the $i$-th view during inference. Notice that in the fixed-view method, the 1st view is selected during training, hence we can observe the result in column 1 is much better than the other columns for fixed-view method. On the contrary, no matter which view is used in inference, the method trained using randomly-selected views can always produce satisfying and consistent results.}
    \label{fig:supp-rot-inv}
\end{figure*}



\section{Low CLIP Similarity on Highly-matched Image-Text Pairs}
\label{sec:supp-clip-sim}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{images/supplementary/clip.png}
    \caption{Result of some clip embedding cosine similarity of text description and image in our train set. Semantically highly matched pairs are placed on the diagonal. 
    }
    \label{fig:low_clip_similarity_on_match_scenes}
    % \vspace{-0.2in}
\end{figure}
As we have mentioned in Sec.\ 3.2, %~\cref{sec:method-pipeline}
although CLIP~\cite{radford2021learning} effectively maps texts and images onto the same space, semantically highly matched image and text pairs still receive low (typically around 30\% to 40\%) cosine similarity, hence making it unlikely for our model trained on pure image embeddings to receive text embeddings directly during inference stage.

We noticed that some prior works such as \cite{Gonsalves_2023} have already demonstrated and discussed such a phenomenon, and in this section, we prove that this holds true on our dataset as well. \Cref{fig:low_clip_similarity_on_match_scenes} shows some examples of image and text pairs, where the cosine similarities of each pair are calculated and displayed in a heat map. We may observe that the pairs on the diagonal are semantically highly matched, yet only receive similarities of around 30\%.



\section{Implementation Details}
\label{sec:supp-impl-detail}

This section provides more implementation details of our model, as an extension of Sec.\ 4.2. %~\cref{sec:implementation}

\noindent \textbf{VAE implementation detail} 
As detailed in Sec.\ 3.2, our NeRF network employs 14 distinct tokens for representation. To facilitate this, we employ 14 independent Variational Autoencoders (VAEs) ~\cite{kingma2013auto} to learn a separate implicit latent space for each token. Each VAE is comprised of an encoder and a decoder, each of which is composed of a 3-layer Multilayer Perceptron (MLP). Two linear layers are added between each encoder and decoder to learn a mean $\boldsymbol{\mu}$ and variance $\boldsymbol{\Sigma}$ for each token, thereby emulating a Gaussian distribution $X \sim \mathcal{N}(\boldsymbol{\mu}, \boldsymbol{\Sigma})$ representing each implicit latent space, subsequently samples an input to the decoder.

\noindent \textbf{Semantic Alignment implementation detail}
We utilized the Transformer~\cite{vaswani2023attention} model to attain semantic alignment, where we regard the semantic clip embedding ${\bf c}\in \mathbb{R}^d$ as the source sequence and its corresponding NeRF parameter in our pretrained latent space ${\bf z}\in \mathbb{R}^{14\times d}$ as the target sequence. In the training phase, a zero-valued beginning-of-sequence ([BOS]) token is appended before the target sequence, and the prediction is performed sequentially. During the inference stage, akin to the training phase, only a zero-valued [BOS] token is provided at the beginning as the target sequence. The Transformer model predicts the next target token based on the provided target sequence (only [BOS] at this stage) and the source sequence. The predicted token is then concatenated after the previous target sequence, and the Transformer model continues to predict the next token, and this process is repeated until all 14 target sequence tokens have been predicted.






% \section{?? More Results for In-distribution Inference}
% \label{sec:supp-more-eg-in-dist}

% {\color{red}Do we need this?}



\section{More Results for Out-of-distribution Inference}
\label{sec:supp-more-eg-ood}

In this section, we provide more out-of-distribution inference results, from both image and text prompts, as an extension to Tab.\ 3 in main paper. %~\cref{tab:out-dist-text-prompt-compare}

\Cref{tab:more-eg-ood-img} shows four more out-of-distribution inference results from image prompts that fall out of our eight categories, and~\cref{tab:more-eg-ood-text} shows four corresponding results from text prompts. We can observe the 3 to 5 times significant acceleration that our initialization brings to the baseline models, either Zero-1-to-3 ~\cite{liu2023zero1to3} for the image-to-NeRF task or DreamFusion ~\cite{poole2022dreamfusion} for the text-to-NeRF task.


\begin{table*}[ht]
    \newcommand{\dummyImg}{\fbox{\rule{0pt}{0.7in} \rule{0.7\linewidth}{0pt}} }
    \centering
    \begin{tabular}{>{\centering\arraybackslash}m{0.13\linewidth}|>{\centering\arraybackslash}m{0.15\linewidth}|>{\centering\arraybackslash}m{0.15\linewidth}|>{\centering\arraybackslash}m{0.15\linewidth}|>
    {\centering\arraybackslash}m{0.15\linewidth}|>
    {\centering\arraybackslash}m{0.15\linewidth}}
    \toprule
        % image table title
        \multirow{2}{*}{Prompt} & Ours & Zero-1-to-3 (S) & Zero-1-to-3 (P) & Zero-1-to-3 (S) & Zero-1-to-3 (P)\\
         & (converge) & (same iterations) & (same iterations) & (converge) & (converge) \\
    \midrule
        % image inference example 1
        \vspace{0.2in}  % center align
        \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/nikon_camera_prompt.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/nikon_combined.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/nikon_ep0126_scratch.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/nikon_ep0126_pretrain.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/nikon_ep0412_scratch_converge.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/nikon_ep0400_pretrain_converge.png}\\
        % image inference example 1 metrics
         & Similarity: 69.6\% & Similarity: 68.1\% & Similarity: 71.3\% & Similarity: 68.4\% & Similarity: 68.3\%\\
         % & SSIM: 77.0\% & SSIM: 77.6\% & SSIM: 80.3\% & SSIM: 76.6\% & SSIM: 86.6\%\\
         % & MS-SSIM: 70.8\% & MS-SSIM: 70.8\% & MS-SSIM: 78.4\% & MS-SSIM: 70.4\% & MS-SSIM: 91.7\%\\
         & Iterations: 12.6k & Iterations: 12.6k & Iterations: 12.6k & Iterations: 41.2k & Iterations: 40k\\\hline

        % image inference example 2
        \vspace{0.2in}  % center align
        \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/iphone_prompt.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/iphone_combined.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/iphone_ep0040_scratch.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/iphone_ep0040_pretrain.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/iphone_ep0200_scratch_converge.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/iphone_ep0179_pretrain_converge.png}\\
        % image inference example 2 metrics
         & Similarity: 93.5\% & Similarity: 84.0\% & Similarity: 90.1\% & Similarity: 92.0\% & Similarity: 92.9\%\\
         % & SSIM: 68.1\% & SSIM: 65.2\% & SSIM: 68.3\% & SSIM: 67.7\% & SSIM: 68.6\%\\
         % & MS-SSIM: 75.3\% & MS-SSIM: 65.0\% & MS-SSIM: 74.5\% & MS-SSIM: 75.8\% & MS-SSIM: 74.4\%\\
         & Iterations: 4k & Iterations: 4k & Iterations: 4k & Iterations: 20k & Iterations: 17.9k\\\hline

         % image inference example 3
        \vspace{0.2in}  % center align
        \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/white_podium.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/podium_combined.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/podium_ep0069_scratch.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/podium_ep0069_pretrain.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/podium_ep0201_scratch_converge.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/podium_ep0212_pretrain_converge.png}\\
        % image inference example 3 metrics
         & Similarity: 85.8\% & Similarity: 78.6\% & Similarity: 74.1\% & Similarity: 81.7\% & Similarity: 86.3\%\\
         % & SSIM: 77.0\% & SSIM: 77.6\% & SSIM: 80.3\% & SSIM: 76.6\% & SSIM: 86.6\%\\
         % & MS-SSIM: 70.8\% & MS-SSIM: 70.8\% & MS-SSIM: 78.4\% & MS-SSIM: 70.4\% & MS-SSIM: 91.7\%\\
         & Iterations: 6.9k & Iterations: 6.9k & Iterations: 6.9k & Iterations: 20.1k & Iterations: 21.2k\\\hline

        % image inference example 4
        \vspace{0.2in}  % center align
        \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/backpack.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/backpack_combined.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/backpack_ep0107_scratch.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/backpack_ep0107_pretrain.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/backpack_ep0347_scratch_converge.png}
        & \includegraphics[width=0.82\linewidth]{images/supplementary/more-ood-image/backpack_ep0334_pretrain_converge.png}\\
        % image inference example 4 metrics
         & Similarity: 94.8\% & Similarity: 89.7\% & Similarity: 90.3\% & Similarity: 94.1\% & Similarity: 93.8\%\\
         % & SSIM: 68.1\% & SSIM: 65.2\% & SSIM: 68.3\% & SSIM: 67.7\% & SSIM: 68.6\%\\
         % & MS-SSIM: 75.3\% & MS-SSIM: 65.0\% & MS-SSIM: 74.5\% & MS-SSIM: 75.8\% & MS-SSIM: 74.4\%\\
         & Iterations: 10.7k & Iterations: 10.7k & Iterations: 10.7k & Iterations: 34.7k & Iterations: 33.4k\\
    \bottomrule
    \end{tabular}
    \caption{More examples of {\bf out-of-distribution inference result, using  image prompts}. For each prompt, we record the convergence iteration count using our initialization zero-shot, from one single forward pass (top-right inset). Scratch (S) or pre-trained (P) Zero-1-to-3 are respectively trained for the same number of iterations and until convergence with their respective results displayed above.
    Our method significantly accelerates the Zero-1-to-3's optimization, achieving 3 to 5 times speed boost while almost consistently yielding better results. Moreover, our method provides a semantically meaningful initialization, as pretrained (P) Zero-1-to-3 still takes an extremely long time to converge though initialized with a similar scene.}
    \label{tab:more-eg-ood-img}
    \vspace{-0.2in}
\end{table*}



\begin{table*}[ht]
    \newcommand{\dummyImg}{\fbox{\rule{0pt}{0.7in} \rule{0.7\linewidth}{0pt}} }
    \centering
    \begin{tabular}{>{\centering\arraybackslash}m{0.13\linewidth}|>{\centering\arraybackslash}m{0.15\linewidth}|>{\centering\arraybackslash}m{0.15\linewidth}|>{\centering\arraybackslash}m{0.15\linewidth}|>
    {\centering\arraybackslash}m{0.15\linewidth}|>
    {\centering\arraybackslash}m{0.15\linewidth}}
    \toprule
        % text table title
        \multirow{2}{*}{Prompt} & Ours & DreamFusion (S) & DreamFusion (P) & DreamFusion (S) & DreamFusion (P)\\
         & (converge) & (same iterations) & (same iterations) & (converge) & (converge) \\
    \midrule
        % % text inference example 1
        % \vspace{0.25in}  % center align
        % {\it ``A yellow sunflower.''}  
        % & \dummyImg
        % & \dummyImg
        % & \dummyImg
        % & \dummyImg
        % & \dummyImg\\
        % % text inference example 1 metrics
        %  & Similarity: 60\% & Similarity: 60\% & Similarity: 60\% & Similarity: 60\% & Similarity: 60\%\\
        %  & Iterations: 10 s & Iterations: 30 min & Iterations: 2 hr & Iterations: 2 hr & Iterations: 2 hr\\\hline

        % text inference example 2
        \vspace{0.25in}  % center align
        {\it ``A colorful Boeing passenger plane.''}  
        & \includegraphics[width=0.75\linewidth]{images/supplementary/more-ood-text/boeing-nrs-75-inset.png}
        & \includegraphics[width=0.75\linewidth]{images/supplementary/more-ood-text/boeing-scratch-75.png}
        & \includegraphics[width=0.75\linewidth]{images/supplementary/more-ood-text/boeing-pretrain-75.png}
        & \includegraphics[width=0.75\linewidth]{images/supplementary/more-ood-text/boeing-scratch-300.png}
        & \includegraphics[width=0.75\linewidth]{images/supplementary/more-ood-text/boeing-pretrain-315.png}\\
        % text inference example 2 metrics
         & Similarity: 31.5\% & Similarity: 29.6\% & Similarity: 28.6\% & Similarity: 33.6\% & Similarity: 33.6\%\\
         & Iterations: 7.5k & Iterations: 7.5k & Iterations: 7.5k & Iterations: 30k & Iterations: 31.5k\\\hline

        % text inference example 3
        \vspace{0.25in}  % center align
        {\it ``Iron man on a blue chair.''}  
        & \vspace{0.05in} \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/ironman-nrs-5k-inset.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/ironman-scratch-5k.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/ironman-pretrain-50.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/ironman-scratch-40k.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/ironman-pretrain-155.png}\\
        % text inference example 3 metrics
         & Similarity: 28.9\% & Similarity: 23.4\% & Similarity: 26.1\% & Similarity: 23.2\% & Similarity: 31.0\%\\
         & Iterations: 5k & Iterations: 5k & Iterations: 5k & Iterations: 40k & Iterations: 15.5k\\\hline

         % text inference example 4
        \vspace{0.25in}  % center align
        {\it ``A burning torch.''}  
        & \vspace{0.05in} \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/torch-nrs-7k-inset.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/torch-scratch-7k.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/torch-pretrain-70.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/torch-scratch-30k.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/torch-pretrain-190.png}\\
        % text inference example 4 metrics
         & Similarity: 32.2\% & Similarity: 30.1\% & Similarity: 29.7\% & Similarity: 32.3\% & Similarity: 31.4\%\\
         & Iterations: 7k & Iterations: 7k & Iterations: 7k & Iterations: 30k & Iterations: 19k\\\hline

         % text inference example 5
        \vspace{0.25in}  % center align
        {\it ``A basketball.''}  
        & \vspace{0.05in} \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/basket-nrs-74-inset.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/basket-scratch-74.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/basket-pretrain-74.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/basket-scratch-180.png}
        & \includegraphics[width=0.72\linewidth]{images/supplementary/more-ood-text/basket-pretrain-195.png}\\
        % text inference example 5 metrics
         & Similarity: 30.4\% & Similarity: 26.1\% & Similarity: 24.1\% & Similarity: 27.3\% & Similarity: 27.4\%\\
         & Iterations: 7.4k & Iterations: 7.4k & Iterations: 7.4k & Iterations: 18k & Iterations: 19.5k\\
    \bottomrule
    \end{tabular}
    \caption{More examples of {\bf out-of-distribution inference result, using text prompts}. For each prompt, we record the convergence iteration count using our initialization zero-shot, from one single forward pass (top-right inset). Scratch (S) or pre-trained (P) DreamFusion are respectively trained for the same number of iterations and until convergence, with their respective results  displayed above.
    Our method significantly accelerates the DreamFusion's optimization, achieving  3 to 5 times speed boost while almost consistently yielding better results. Moreover, our method provides a semantically meaningful initialization, as pretrained (P) DreamFusion still takes an extremely long time to converge though initialized with a similar scene.}
    \label{tab:more-eg-ood-text}
    \vspace{-0.2in}
\end{table*}





\section{Interpolation Results}
\label{sec:supp-interpolation}

We continue the discussion in Sec.\ 4.6 %~\cref{sec:results-outdomain}
to demonstrate that our method has learned a semantically meaningful alignment by displaying some interpolation results, thereby providing a valid explanation of why the initializations given by our method yield much faster convergence compared with the pre-trained baseline (P), which is also trained to a semantically close scene.
The results in~\cref{fig:interpolation} demonstrate that we can get not only smooth interpolation between objects with a single feature, like colors, but also a smooth morph between two objects with a difference in both geometry and color. (Video results presented in the same directory of this file)

\begin{figure*}
    \centering
    \includegraphics[width=0.48\linewidth, trim={2cm 2cm 2cm 2cm},clip]{images/supplementary/interpolation/65f163_7c16a2.png}
    \includegraphics[width=0.48\linewidth, trim={2cm 2cm 2cm 2cm},clip]{images/supplementary/interpolation/7c16a2_28fb62.png}
    \caption{Interpolation results, with two objects differ only in color (left) and differ both in color and shape (right). Each time we slightly increase the weight of the first object for interpolation, decrease the weight of the second object by 0.01, and organize the results row by row, which allows us to observe a smooth interpolation result.}
    \label{fig:interpolation}
\end{figure*}
% \section{More Results for Initialization Methods Comparison}
% \label{sec:supp-init-method}

% Here, we provide the remaining eight comparison results on different NeRF initialization methods, as mentioned in Sec.\ 5.2.%~\cref{sec:ablation-how-to-init}



\section{Comparisons on Convergence Speed}
\label{sec:supp-converge-curve}

As previous results only provide the number of iterations required for convergence when demonstrating the effective acceleration ability of our initialization, here we include examples of the curves comparing the optimization process of the baseline model (Zero-1-to-3 for image-to-NeRF tasks and DreamFusion for text-to-NeRF tasks) with/without our initialization.

Specifically, after training every 100 iterations (or one epoch), we render $m$ images $I_{1}^{(i)}, I_{2}^{(i)}, \cdots, I_{m}^{(i)}$ for epoch $i$, from viewpoints evenly divided from $360^\circ$, and compute the pixel-wise mean-squared difference $D_i$ between the $m$ images rendered in the $i$-th epoch and the previous $(i-1)$-th epoch. This metric can be formulated as
\begin{align*}
    D_i &= \sum_{j=1}^{m} \left\| I_{j}^{(i)} - I_{j}^{(i-1)} \right\|_2^2,\quad {\rm for\ } i > 1\\
    % D_1 &= \sum_{j=1}^{m} \left\| I_{j}^{(i)} \right\|_2^2
    D_1 &= 0
\end{align*}
where by taking the difference of two images $I$ we mean the pixel-wise difference.

We then consider the optimization process is converged if
$D_i<\epsilon$ for continuous $20$ epochs.

\Cref{fig:supp-converge-curve} shows two examples of the convergence curves with $m=8$ and $\epsilon=0.01$, using image prompt and text prompt, respectively. We may clearly observe the acceleration that our initialization brings to the baseline.
% We further include the changes in cosine similarity, demonstrating that our method converges faster to a (normally) higher similarity score.

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{images/supplementary/converge-curve/converge-curve-image-bird-loss.png}
    % \includegraphics[width=0.48\textwidth]{images/supplementary/converge-curve/converge-curve-image-bird-sim.png}
    \includegraphics[width=0.48\textwidth]{images/supplementary/converge-curve/converge-curve-text-boeing-loss.png}
    % \includegraphics[width=0.48\textwidth]{images/supplementary/converge-curve/converge-curve-image-bird-sim.png}
    \caption{Comparisons of optimization convergence curves with (Ours) / without (DreamFusion) our initialization, when using image (left) and text (right) prompts for inference.}
    \label{fig:supp-converge-curve}
\end{figure*}




\section{Video \& Multi-view Results of Generated Scenes}
\label{sec:supp-video}

In this section, we provide some video results of the NeRF scene we generated, as well as the 8 multi-view images used to generate the videos, demonstrating that our implicit generation method yields satisfying view-consistent NeRF scenes.

We randomly select some samples from our test split and display them in~\cref{fig:supp-multi-view-in-dist-1,fig:supp-multi-view-in-dist-2}. For out-of-distribution image or text inference results, we display them in~\cref{fig:supp-multi-view-out-dist-img} and~\cref{fig:supp-multi-view-out-dist-text}, respectively. The videos can be found in the same directory of this file.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_5c1766b6586f451cb61df9fa29d3914e.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/bathtub_cd23523044b34cb29a461ceb2370bcba.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/car_b05d651c17e9e626ca92a4cdad802b45.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_28fb62e117f94307b30562497d49fc73.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_6abe62bea98941edbc6209fe95ff0f43.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/car_65c225fae513a6dbe7b23463fd9b0ba1.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_ff2f975a23b78bc78caa71b1fbf7fb98.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_7c16a2039b954637b4a7764f1b9f64b5.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/bathtub_2a28b3c0318590983c8d0fdfb1cc2535.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/laptop_5fb5b09b324dc153ed883f1f11a51185.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_542a1e7f0009339aa813ec663952445c.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/guitar_887c39981c4cfef661cdd121f4738c70.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_65f16361919f4901a3fa3679e7ca9e09.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_d777b1e4ba72cebac5353b0f3cdec54.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/bathtub_e78f7e89878402513af30a3946d92feb.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/lamp_8e2c822e2a316fa04f3443b22038d340.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/guitar_5c805aca7aa8bdd3ac61a2f8346a8f.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_0981a5c30fdf4416ab03bd6e32a77d08.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/laptop_f496fa98fb41f6b1ea5768960d4a805c.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_26237deeb192f83d3ada73811bb576de.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/car_d9867d92edba3d0cb96212c8f6cd06e.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/lamp_2a5e2e5ec5eb986385bf3590978fc71f.png}
    \caption{{\bf Multi-view results of in-distribution inference from image prompts}.
    Samples are randomly selected from our test split. For each scene, we display the 8 camera views generated by our NeRF obtained.}
    \label{fig:supp-multi-view-in-dist-1}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_ccea7e2e68c943b6b85cdb93fd9898f2.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/guitar_4e982d5baec36536c86b22832615248.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_c2e38200a238177ebbf3143b1cb6076a.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/car_8fc220461ea512f3abeba927b56dd398.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/train_a10330472393343e44399be51ebd0ad9.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_2f1ba13a0dcd4e8f96ff20a408f0e2d1.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/lamp_64f61c9c81e3eb7b8aaae3d020f5ddf8.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_f1210d8f895e40b663c15773e7567372.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_ff2f975a23b78bc78caa71b1fbf7fb98.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_5c1766b6586f451cb61df9fa29d3914e.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_bdf120e29b19f77b352526271bef32d2.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/lamp_9d66a6faebd46b1d68661782af60b711.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/train_6f4ac6a0940302a31307b8e7d9f7be90.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_42b63c881861105ccc14f1e6f4f4f49b.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/laptop_90c01fd78513bb99c9b20aa1b8066c46.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_acd8ae7c85044c74abf8514b977deb65.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/guitar_c0dc0328e787d4795c0be177939e290.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/bathtub_f8d0cc0680f502e98eb3bc6c6d15f9bf.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/chair_0144133a874d4fa9881d8947928999e0.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/plane_7315cd530e4858246ed10e8f7fe336e.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/car_8c1b20c4c37dc679301fa882a9655049.png}
    \includegraphics[width=0.49\linewidth,trim={2cm 2cm 0 0},clip]{images/supp-in-dist-images/guitar_73a1ac3658e2505f76d05024fabfa1e5.png}
    \caption{({\it Cont.}) {\bf Multi-view results of in-distribution inference from image prompts}.}
    \label{fig:supp-multi-view-in-dist-2}
\end{figure*}

% \begin{figure*}[ht]
%     \centering
    
%     \caption{({\it Cont.}){\bf Multi-view results of in-distribution inference from image prompts}.}
%     \label{fig:supp-multi-view-in-dist-3}
% \end{figure*}





%% ood multi-view
\begin{figure*}[ht]
    \centering
    % bird
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/bird-view_1_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/bird-view_2_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/bird-view_3_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/bird-view_4_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/bird-view_5_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/bird-view_6_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/bird-view_7_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/bird-view_8_.png}\\
    % briefcase
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/briefcase-view_1_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/briefcase-view_2_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/briefcase-view_3_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/briefcase-view_4_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/briefcase-view_5_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/briefcase-view_6_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/briefcase-view_7_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/briefcase-view_8_.png}\\
    % iPhone
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/iphone-view_1_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/iphone-view_2_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/iphone-view_3_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/iphone-view_4_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/iphone-view_5_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/iphone-view_6_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/iphone-view_7_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/iphone-view_8_.png}\\
    % podiumiphone
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/podium-view_1_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/podium-view_2_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/podium-view_3_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/podium-view_4_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/podium-view_5_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/podium-view_6_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/podium-view_7_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/podium-view_8_.png}
    \caption{{\bf Multi-view results of out-of-distribution inference from image prompts}.
    We reuse the samples shown in the experiment results section in out-of-distribution inference. We display the 8 camera views generated by our NeRF obtained for each scene. Prompts used are the same in previous experiment results.}
    \label{fig:supp-multi-view-out-dist-img}
\end{figure*}

\begin{figure*}[ht]
    \centering
    % brown table
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/brown-table-view_1_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/brown-table-view_2_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/brown-table-view_3_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/brown-table-view_4_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/brown-table-view_5_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/brown-table-view_6_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/brown-table-view_7_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/brown-table-view_8_.png}\\
    % boeing
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/boeing-view_1_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/boeing-view_2_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/boeing-view_3_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/boeing-view_4_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/boeing-view_5_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/boeing-view_6_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/boeing-view_7_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/boeing-view_8_.png}\\
    % basketball
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/basketball-view_1_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/basketball-view_2_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/basketball-view_3_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/basketball-view_4_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/basketball-view_5_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/basketball-view_6_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/basketball-view_7_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/basketball-view_8_.png}\\
    % torch
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/torch-view_1_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/torch-view_2_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/torch-view_3_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/torch-view_4_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/torch-view_5_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/torch-view_6_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/torch-view_7_.png}
    \includegraphics[width=0.12\textwidth]{images/supplementary/multiview-ood/torch-view_8_.png}
    \caption{{\bf Multi-view results of out-of-distribution inference from text prompts}.
    We reuse the samples shown in the experiment results section in out-of-distribution inference. We display the 8 camera views generated by our NeRF obtained for each scene. Prompts used (from top to bottom): ``A brown table.'', ``A colorful Boeing passenger plane.'', ``A basketball.'', ``A burning torch.''}
    \label{fig:supp-multi-view-out-dist-text}
\end{figure*}

==> sec/X_suppl_template.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary


\section{Rationale}
\label{sec:rationale}
% 
Having the supplementary compiled together with the main paper means that:
% 
\begin{itemize}
\item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
\item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
\item When submitted to arXiv, the supplementary will already included at the end of the paper.
\end{itemize}
% 
To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.
